CyCNN: A Rotation Invariant CNN using Polar Mapping and Cylindrical Convolution Layers

Deep Convolutional Neural Networks (CNNs) are empirically known to be invariant to moderate translation but not to rotation in image classification. This paper proposes a deep CNN model, called CyCNN, which exploits polar mapping of input images to convert rotation to translation. To deal with the cylindrical property of the polar coordinates, we replace convolution layers in conventional CNNs to cylindrical convolutional (CyConv) layers. A CyConv layer exploits the cylindrically sliding windows (CSW) mechanism that vertically extends the input-image receptive fields of boundary units in a convolutional layer. We evaluate CyCNN and conventional CNN models for classification tasks on rotated MNIST, CIFAR-10, and SVHN datasets. We show that if there is no data augmentation during training, CyCNN significantly improves classification accuracies when compared to conventional CNN models. Our implementation of CyCNN is publicly available on https://github.com/mcrl/CyCNN.

==> implementation.tex <==
\section{Implementation}
We use PyTorch~\cite{NEURIPS2019_9015} library to implement and evaluate models. We manually implement \textsf{CyConv} layers using CUDA~\cite{cuda} to train CyCNN models on GPUs. We integrate our CUDA kernels into PyTorch source code. We use OpenCV~\cite{opencv_library} library to implement image rotation and the polar coordinate conversion. 

\subsection{Cylindrical Winograd Convolution}
While our manually-implemented CUDA kernels are functionally correct, those kernels are too slow compared to cuDNN~\cite{cudnn} non-cylindrical convolution primitives. For instance, when we convert convolution layers of VGG19~\cite{SIZI-ICLR-2015} to \textsf{CyConv} layers, the elapsed time for training one epoch becomes $20\times$ larger.  

When we use the \textsf{CyWino} layer, still, training one epoch for VGG19 is $1.45\times$ slower than the cuDNN-based baseline. However, this is not because \textsf{CyConv} algorithm is inefficient, but because cuDNN is highly optimized compared to our implementation. We manually implement the Winograd convolution layer as well, and observe that the performance of it is the same as that of \textsf{CyConv} layer. This implies our techniques can be integrated into other highly-optimized GPU kernels (e.g.,cuDNN) without additional overheads.


